Bias in Machine Learning Software: Why? How? What to do?

Increasingly, software is making autonomous decisions in case of criminal sentencing, approving credit cards, hiring employees, and so on. Some of these decisions show bias and adversely affect certain social groups (e.g. those defined by sex, race, age, marital status). Many prior works on bias mitigation take the following form: change the data or learners in multiple ways, then see if any of that improves fairness. Perhaps a better approach is to postulate root causes of bias and then applying some resolution strategy. This paper postulates that the root causes of bias are the prior decisions that affect- (a) what data was selected and (b) the labels assigned to those examples. Our Fair-SMOTE algorithm removes biased labels; and rebalances internal distributions such that based on sensitive attribute, examples are equal in both positive and negative classes. On testing, it was seen that this method was just as effective at reducing bias as prior approaches. Further, models generated via Fair-SMOTE achieve higher performance (measured in terms of recall and F1) than other state-of-the-art fairness improvement algorithms. To the best of our knowledge, measured in terms of number of analyzed learners and datasets, this study is one of the largest studies on bias mitigation yet presented in the literature.

==> options.tex <==
\begin{table}

%\captionsetup{font=footnotesize}
\caption{Hyperparameter  options
seen in recent SE papers~\cite{ghotra2015revisiting,fu2016tuning,agrawal2018better,agrawal2018wrong} and in  the documentation of a widely-used data mining library
(Scikit-learn~\cite{pedregosa2011scikit}) for a list of options not explored
in those studies.
While this list is incomplete, it does include many
of the   hyperparameter optimizations being explored in the literature. }\label{tbl:options}
\footnotesize
 
\begin{tabular}{|p{.95\linewidth}|}\hline
\textbf{Learners:}  


\noindent
\bi
\item DecisionTreeClassifier(criterion=b, splitter=c, min\_samples\_split=a)
    \bi
   \item a, b, c= randuniform(0.0,1.0), randchoice([`gini',`entropy']), \newline randchoice([`best',`random'])
   \ei
\item RandomForestClassifier(n\_estimators=a,criterion=b,  min\_samples\_split=c)
    \bi
   \item a,b,c = randint(50, 150), randchoice(['gini', 'entropy']),\newline randuniform(0.0, 1.0) 
   \ei
\item LogisticRegression(penalty=a, tol=b, C=float(c))
    \bi
    \item a,b,c=randchoice([`l1',`l2']), randuniform(0.0,0.1), randint(1,500)
    \ei 
\item MultinomialNB(alpha=a) = randuniform(0.0,0.1)
\item KNeighborsClassifier(n\_neighbors=a, weights=b, p=d, metric=c)
    \bi
    \item a, b,c  = randint(2, 25), randchoice([`uniform', `distance']), \newline randchoice([`minkowski',`chebyshev'])
    \item if c=='minkowski': d= randint(1,15)  else:  d=2
    \ei
     
    
\ei
\\\hline

{\bf Pre-processors for   defect prediction, Issue lifetime, Bad   Smells:} 

\bi 
\item StandardScaler
\item MinMaxScaler
\item MaxAbsScaler
\item RobustScaler(quantile\_range=(a, b)) =  randint(0,50), randint(51,100) 
\item KernelCenterer
\item QuantileTransformer(n\_quantiles=a,  output\_distribution=c, subsample=b)
    \bi
    \item a, b = randint(100, 1000), randint(1000, 1e5)
    \item c = randchoice([`normal',`uniform'])
    \ei
\item Normalizer(norm=a) = randchoice([`l1', `l2',`max'])
  
\item Binarizer(threshold=a) =  randuniform(0,100)
   
    \item SMOTE(a=n\_neighbors, b=n\_synthetics,  c=Minkowski\_exponent)
    \bi
    \item a,b = randit(1,20),randchoice(50,100,200,400)
    \item c = randuniform(0.1,5)
    \ei
\ei

 \\\hline
{\bf Pre-Processors for Text mining:}  
 
\bi
\item CountVectorizer(max\_df=a, min\_df=b) = randint(100, 1000), randint(1, 10)
\item TfidfVectorizer(max\_df=a, min\_df=b, norm=c)
    \bi
    \item a, b,c = randint(100, 1000), randint(1, 10), randchoice([`l1', `l2', None])
    \ei
\item HashingVectorizer(n\_features=a, norm=b)
    \bi
    \item a = randchoice([1000, 2000, 4000, 6000, 8000, 10000])
    \item b = randchoice([`l1', `l2', None])
    \ei
\item LatentDirichletAllocation(n\_components=a, doc\_topic\_prior=b,\newline topic\_word\_prior=c,
                                   learning\_decay=d,
                                   learning\_offset=e,batch\_size=f)
    \bi
    \item a, b, c = randint(10, 50), randuniform(0, 1),  randuniform(0, 1)
    \item d, e  = randuniform(0.51, 1.0), randuniform(1, 50), 
    \item f = randchoice([150,180,210,250,300])
    \ei
\ei 


 \\\hline
 \end{tabular}

\end{table}

==> table5.tex <==
\begin{tabular}{|c|c|c|c|c|c|
>{\columncolor[HTML]{D28986}}c |
>{\columncolor[HTML]{D28986}}c |c|c|c|c|}
\hline
\cellcolor[HTML]{C0C0C0}Dataset                                                  & \cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}c@{}}Protected\\ Attribute\end{tabular} & \cellcolor[HTML]{C0C0C0}Algorithms & \cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}c@{}}Recall\\ (+)\end{tabular} & \cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}c@{}}False\\ alarm\\ (-)\end{tabular} & \cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}c@{}}Precision\\ (+)\end{tabular} & \cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}c@{}}Accuracy\\ (+)\end{tabular} & \cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}c@{}}F1 Score\\ (+)\end{tabular} & \cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}c@{}}AOD\\ (-)\end{tabular} & \cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}c@{}}EOD\\ (-)\end{tabular} & \cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}c@{}}SPD\\ (-)\end{tabular} & \cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}c@{}}DI\\ (-)\end{tabular} \\ \hline
                                                                                 &                                                                                       & Default - LSR                      & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.42}                          & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.07}                                 & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.69}                             & {\color[HTML]{000000} 0.83}                                                    & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.54}                            & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.12}                       & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.24}                       & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.21}                       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.56}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & Default - RF                       & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.51}                          & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.06}                                 & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.72}                             & {\color[HTML]{000000} 0.83}                                                    &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.59}                            &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.09}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.17}                       & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.17}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.33}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & Default - SVM                      & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.35}                          & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.04}                                 & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.81}                             & {\color[HTML]{000000} 0.82}                                                    & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.49}                            & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.1}                        & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.24}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.14}                       & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.43}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & SMOTE - LSR                        & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.70}                          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.25}                                 & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.49}                             & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.70}                            & {\color[HTML]{000000} 0.64}                                                    & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.17}                       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.37}                       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.33}                       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.58}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & SMOTE - RF                         & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.61}                          & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.07}                                 & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.71}                             & {\color[HTML]{000000} 0.83}                                                    & {\color[HTML]{000000} 0.62}                                                    &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.08}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.16}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.16}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.32}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & SMOTE - SVM                        & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.71}                          &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.19}                                 & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.55}                             &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.78}                            & {\color[HTML]{000000} 0.62}                                                    & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.11}                       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.52}                       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.42}                       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.46}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & Fair-SMOTE - LSR                   & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.71}                          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.25}                                 & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.51}                             & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.73}                            & {\color[HTML]{000000} 0.62}                                                    & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.01}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.02}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.03}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.15}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & Fair-SMOTE - RF                    & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.69}                          &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.2}                                  & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.53}                             &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.78}                            & {\color[HTML]{000000} 0.6}                                                     & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.03}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.04}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.1}                        & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.22}                      \\ \cline{3-12} 
\multirow{-9}{*}{\begin{tabular}[c]{@{}c@{}}Adult Census \\ Income\end{tabular}} & \multirow{-9}{*}{Sex}                                                                 & Fair-SMOTE - SVM                   & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.73}                          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.23}                                 & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.51}                             &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.76}                            & {\color[HTML]{000000} 0.6}                                                     & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.02}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.02}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.08}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.21}                      \\ \hline
                                                                                 &                                                                                       & Default - LSR                      & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.42}                          & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.05}                                 & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.69}                             & {\color[HTML]{000000} 0.81}                                                    &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.52}                            &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.06}                       & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.15}                       & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.16}                       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.52}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & Default - RF                       & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.53}                          & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.07}                                 & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.7}                              & {\color[HTML]{000000} 0.83}                                                    & {\color[HTML]{000000} 0.6}                                                     & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.12}                       & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.16}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.12}                       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.57}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & Default - SVM                      & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.35}                          & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.03}                                 & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.8}                              & {\color[HTML]{000000} 0.82}                                                    &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.49}                            & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.08}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.11}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.10}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.35}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & SMOTE - LSR                        & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.71}                          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.23}                                 & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.49}                             &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.72}                            & {\color[HTML]{000000} 0.61}                                                    & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.16}                       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.19}                       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.23}                       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.56}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & SMOTE - RF                         &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.66}                          &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.08}                                 &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.67}                             & {\color[HTML]{000000} 0.83}                                                    & {\color[HTML]{000000} 0.63}                                                    & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.09}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.12}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.12}                       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.52}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & SMOTE - SVM                        & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.58}                          &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.11}                                 &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.62}                             & {\color[HTML]{000000} 0.81}                                                    & {\color[HTML]{000000} 0.6}                                                     & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.09}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.12}                       & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.17}                       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.32}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & Fair-SMOTE - LSR                   & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.7}                           & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.22}                                 & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.51}                             &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.72}                            & {\color[HTML]{000000} 0.62}                                                    & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.04}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.03}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.05}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.26}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & Fair-SMOTE - RF                    & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.73}                          & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.2}                                  & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.52}                             & {\color[HTML]{000000} 0.8}                                                     & {\color[HTML]{000000} 0.61}                                                    & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.01}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.02}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.08}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.29}                      \\ \cline{3-12} 
\multirow{-9}{*}{\begin{tabular}[c]{@{}c@{}}Adult Census \\ Income\end{tabular}} & \multirow{-9}{*}{Race}                                                                & Fair-SMOTE - SVM                   & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.71}                          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.26}                                 & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.5}                              & {\color[HTML]{000000} 0.75}                                                    & {\color[HTML]{000000} 0.61}                                                    & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.01}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.01}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.06}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.18}                      \\ \hline
                                                                                 &                                                                                       & Default - LSR                      & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.73}                          & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.38}                                 & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.66}                             & {\color[HTML]{000000} 0.64}                                                    & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.61}                            &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.05}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.14}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.18}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.24}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & Default - RF                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.75}                          &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.45}                                 & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.66}                             & {\color[HTML]{000000} 0.67}                                                    & {\color[HTML]{000000} 0.72}                                                    & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.11}                       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.18}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.2}                        & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.34}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & Default - SVM                      & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.77}                          &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.45}                                 & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.66}                             & {\color[HTML]{000000} 0.67}                                                    & {\color[HTML]{000000} 0.71}                                                    & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.1}                        &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.15}                       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.22}                       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.28}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & SMOTE - LSR                        & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.65}                          & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.33}                                 &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.62}                             &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.6}                             &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.65}                            & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.08}                       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.19}                       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.22}                       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.31}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & SMOTE - RF                         &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.72}                          &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.42}                                 & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.67}                             & {\color[HTML]{000000} 0.65}                                                    &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.7}                             & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.11}                       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.22}                       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.26}                       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.3}                       \\ \cline{3-12} 
                                                                                 &                                                                                       & SMOTE - SVM                        &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.7}                           & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.36}                                 & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.68}                             & {\color[HTML]{000000} 0.66}                                                    & {\color[HTML]{000000} 0.69}                                                    & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.1}                        & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.21}                       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.31}                       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.38}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & Fair-SMOTE - LSR                   & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.62}                          & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.32}                                 & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.56}                             &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.55}                            &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.65}                            & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.02}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.05}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.08}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.04}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & Fair-SMOTE - RF                    &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.71}                          &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.44}                                 & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.66}                             & {\color[HTML]{000000} 0.65}                                                    & {\color[HTML]{000000} 0.7}                                                     & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.04}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.03}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.1}                        & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.02}                      \\ \cline{3-12} 
\multirow{-9}{*}{Compas}                                                         & \multirow{-9}{*}{Sex}                                                                 & Fair-SMOTE - SVM                   & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.79}                          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.5}                                  & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.65}                             & {\color[HTML]{000000} 0.66}                                                    & {\color[HTML]{000000} 0.71}                                                    & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.02}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.01}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.06}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.08}                      \\ \hline
                                                                                 &                                                                                       & Default - LSR                      & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.69}                          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.39}                                 & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.65}                             & {\color[HTML]{000000} 0.64}                                                    &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.68}                            &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.05}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.11}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.12}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.21}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & Default - RF                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.75}                          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.44}                                 & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.66}                             & {\color[HTML]{000000} 0.66}                                                    & {\color[HTML]{000000} 0.7}                                                     & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.07}                       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.17}                       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.21}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.24}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & Default - SVM                      & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.77}                          & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.45}                                 & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.66}                             & {\color[HTML]{000000} 0.67}                                                    & {\color[HTML]{000000} 0.71}                                                    & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.07}                       & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.14}                       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.18}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.24}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & SMOTE - LSR                        &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.61}                          & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.32}                                 &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.61}                             &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.6}                             &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.63}                            & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.06}                       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.16}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.14}                       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.27}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & SMOTE - RF                         & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.75}                          &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.42}                                 & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.67}                             & {\color[HTML]{000000} 0.66}                                                    & {\color[HTML]{000000} 0.7}                                                     & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.07}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.13}                       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.19}                       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.31}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & SMOTE - SVM                        & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.7}                           &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.39}                                 & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.68}                             & {\color[HTML]{000000} 0.66}                                                    & {\color[HTML]{000000} 0.69}                                                    & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.09}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.12}                       & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.16}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.24}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & Fair-SMOTE - LSR                   &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.62}                          & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.30}                                 &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.56}                             & {\color[HTML]{000000} 0.55}                                                    & {\color[HTML]{000000} 0.66}                                                    & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.01}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.05}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.06}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.11}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & Fair-SMOTE - RF                    &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.66}                          &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.39}                                 & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.67}                             & {\color[HTML]{000000} 0.65}                                                    & {\color[HTML]{000000} 0.67}                                                    & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.01}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.03}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.02}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.10}                      \\ \cline{3-12} 
\multirow{-9}{*}{Compas}                                                         & \multirow{-9}{*}{Race}                                                                & Fair-SMOTE - SVM                   & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.7}                           &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.41}                                 & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.67}                             & {\color[HTML]{000000} 0.65}                                                    & {\color[HTML]{000000} 0.68}                                                    & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.02}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.06}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.08}                       & \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.12}                      \\ \hline
                                                                                 &                                                                                       & Default - LSR                      &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.35}                          &  \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.05}                                 &  \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.65}                             &  \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.85}                            &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.44}                            &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.04}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.1}                        &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.07}                       & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.43}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & Default - RF                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.38}                          &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.11}                                 &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.62}                             &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.81}                            &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.41}                            & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.08}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.12}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.08}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.36}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & Default - SVM                      &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.31}                          &  \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.08}                                 &  \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.66}                             &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.79}                            &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.4}                             & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.09}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.1}                        &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.09}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.32}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & SMOTE - LSR                        &  \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.65}                          & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.22}                                 & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.58}                             &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.78}                            &  \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.49}                            & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.17}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.11}                       & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.11}                       & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.49}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & SMOTE - RF                         &  \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.63}                          & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.18}                                 & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.56}                             &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.78}                            &  \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.52}                            & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.12}                       & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.19}                       & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.13}                       &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.31}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & SMOTE - SVM                        &  \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.62}                          & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.23}                                 & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.49}                             &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.79}                            &  \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.5}                             & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.13}                       & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.18}                       & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.15}                       & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.47}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & Fair-SMOTE - LSR                   &  \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.66}                          & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.2}                                  & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.41}                             &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.77}                            &  \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.51}                            &  \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.01}                       &  \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.03}                       &  \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.04}                       &  \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.17}                      \\ \cline{3-12} 
                                                                                 &                                                                                       & Fair-SMOTE - RF                    &  \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.62}                          & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.21}                                 & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.38}                             &  \cellcolor[HTML]{FFABA7}{\color[HTML]{000000} 0.77}                            &  \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.48}                            &  \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.03}                       &  \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.04}                       &  \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.03}                       &  \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.19}                      \\ \cline{3-12} 
\multirow{-9}{*}{MEPS - 16}                                                      & \multirow{-9}{*}{Sex}                                                                 & Fair-SMOTE - SVM                   &  \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.61}                          & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.18}                                 & \cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.39}                             & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0.76}                            &  \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.49}                            &  \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.04}                       &  \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.03}                       &  \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.05}                       &  \cellcolor[HTML]{D28986}{\color[HTML]{000000} 0.19}                      \\ \hline
\end{tabular}
